Layout decomposition for triple patterning lithography

As minimum feature size and pitch spacing further decrease, triple patterning lithography (TPL) is a possible 193nm extension along the paradigm of double patterning lithography (DPL). However, there is very little study on TPL layout decomposition. In this paper, we show that TPL layout decomposition is a more difficult problem than that for DPL. We then propose a general integer linear programming formulation for TPL layout decomposition which can simultaneously minimize conflict and stitch numbers. Since ILP has very poor scalability, we propose three acceleration techniques without sacrificing solution quality: independent component computation, layout graph simplification, and bridge computation. For very dense layouts, even with these speedup techniques, ILP formulation may still be too slow. Therefore, we propose a novel vector programming formulation for TPL decomposition, and solve it through effective semidefinite programming (SDP) approximation. Experimental results show that the ILP with acceleration techniques can reduce 82% runtime compared to the baseline ILP. Using SDP based algorithm, the runtime can be further reduced by 42% with some tradeoff in the stitch number (reduced by 7%) and the conflict (9% more). However, for very dense layouts, SDP based algorithm can achieve 140x speed-up even compared with accelerated ILP.

==> doc/SDP_useless.tex <==
Consider the following vector programming, which simultaneously minimize conflict number and stitch number.
In other words, it is equivalent to equation (\ref{eq:math}).
We have a $m$-dimensional unit vector $v_i$ for each node $i$: 

\begin{align}
    \label{eq:SDP1}
    \textrm{min}  & \sum_{e_{ij} \in CE}  ( v_i \cdot v_j + \frac{1}{2} ) + \alpha \sum_{e_{ij} \in SE} ( 1 - v_i \cdot v_j ) \ \  \tag{$III$}\\
    \textrm{s.t}.\ \ 	&   v_i \cdot v_j \ge - \frac{1}{2}, \ \ \	\forall e_{ij} \in CE 		&\tag{$IIIa$}\\
            			& v_i \cdot v_i = 1 , \ \ \                   		\forall i \in V			&\tag{$IIIb$}\\
				& v_i \cdot v_j \le 1	, \ \ \			\forall e_{ij} \in SE		&\tag{$IIIc$}
\end{align}

\begin{align}
    \label{eq:SDP2}
    \textrm{min}  & \sum_{e_{ij} \in CE}  ( v_i \cdot v_j + \frac{1}{2} ) + \alpha \sum_{e_{ij} \in SE} ( 1 - v_i \cdot v_j ) \ \  \tag{$III$}\\
    \textrm{s.t}.\ \ 	& v_i \cdot v_i = 1 , \ \ \                   		\forall i \in V			&\tag{$IIIa$}
\end{align}


The object function is try to minimize conflicts, because if $i$ and $j$ are assigned the same color,
$v_i \cdot v_j$ contributes $1$ to the objective function, and $0$ otherwise.
%The number of conflicts can be formulated as follow:


\subsection{K-Coloring Matrix (Useless)}

Given a graph $G=(V, E)$, we define two concepts: vector $k$-coloring and matrix $k$-coloring.
In this section we write the inner product of $v_i$ and $v_j$ as $v_i \cdot v_j$, or sometimes as $v_i^Tv_j$.

\begin{define}[Vector $k$-coloring]
A vector $k$-coloring of $G$ is an assignment of unit vector $v_i$ from the space $R^n$ to each vertex $i \in V$, such that for any two adjacent vertices $i$ and $j$ the inner product of their vectors satisfies the inequality $v_i \cdot v_j \le \frac{-1}{k-1}$.
\end{define}


\begin{define}[Matrix $k$-coloring]
A matrix $k$-coloring of $G$ is an $n \times n$ symmetric positive semidefinite matrix $M$, with $m_{ii}=1$ and $m_{ij} \le \frac{-1}{k-1}$ if $e_{ij} \in E$.
\end{define}

We will show that matrix and vector $k$-colorings are in fact equivalent.
Thus, to solve the vector coloring relaxation, it will suffice to find a matrix $k$-coloring.

\begin{lemma}
\label{lem:equal}
A graph has a vector $k$-coloring if and only if it has matrix $k$-coloring.
\end{lemma}

\begin{proof}
Given a vector $k$-coloring $\{v_i\}$, the matrix $k$-coloring is defined by $m_{ij}=v_i \cdot v_j$.
For the other direction, it is well known that for every symmetric positive definite matrix $M$, by Cholesky decomposition there exists a square matrix $U$ such that $UU^T = M$. The rows of $U$ are vectors $\{u_i\}$ that form a vector $k$-coloring of $G$.
\end{proof}

\begin{theorem}
Every $k$-colorable graph $G$ has a vector $k$-coloring.
\end{theorem}


Using the Cholesky Decomposition, we finally get the following matrix $V$ whose rows are the vectors assigned to each node of the graph.
Note that $X = V V^T$.
\begin{displaymath}
	V =
	\left(
		\begin{array}{c}
			v_1\\ v_2\\ v_3\\ v_4\\ v_5
		\end{array}
	\right) = 
	\left(
		\begin{array}{ccccc}
			0.019&	-0.5&	-0.866&	0&	0\\
			0.039&	0.99&	0&		0&	0\\
			0.019&	-0.5&	0.866&	0&	0\\
			0.019&	-0.5&	-0.866&	0&	0\\
			0.019&	-0.5&	0.866&	0&	0\\
		\end{array}
	\right)
\end{displaymath}

The next step contains the randomness of the algorithm. 
We choose a random vector $r = \{r_1, r_2, \cdots, r_5\}$ by drawing each $r_i$ independently from the standard normal distribution $\boldmath N(0,1)$. For example, we randomly choose $r$ as follow:
\begin{displaymath}
	r = \{0.087, -0.159, 0.284, -0.309, -0.166\}
\end{displaymath}

For each $v_i$, by calculating $v_i = v_i \cdot r$, we get following vector:
\begin{displaymath}
	v = (-0.165, -0.154, 0.327, -0.165, 0.327)
\end{displaymath} 
After sorting, we can get this order: $(v_3, v_5, v_1, v_4, v_2)$.
Using Algorithm \ref{alg:Rounding}, we can assign node 3 and node 5 with first color.
Then we remove node 3 and node 5 in decomposition graph, and simplified graph is shown in Fig. \ref{fig:example}(c).
On the simplified decomposition graph, since we only assign all nodes two color, Graph Reduction based ILP algorithm \cite{DPL_ICCAD09_Xu} or any other decomposition algorithm in Double Patterning can be adopted directly.



\begin{algorithm}[htb]
\caption{Rounding Algorithm for vector programming} 
\label{alg:Rounding}
\begin{algorithmic}[1]
	%\REQUIRE vector $v_i$ solved by vector programming (\ref{eq:SDP1}) or (\ref{eq:SDP2}).
	\STATE Solve program (\ref{eq:sdp}), get matrix $X$.
	\STATE Draw random vector $r$.
	\FORALL{$v_i$ in $\{v\}$}
		\STATE $v_i = v_i \cdot r$.
	\ENDFOR
	\STATE sort($\{v\}$).
	\FOR{$i=1$ to $\{v\}.size()$}
		%\IF{$v_i$ is legal}
		\IF{$\forall e_{ij} \in CE$ or $SE$, $v_j \notin S$}
			\STATE $S \leftarrow v_i$.
		\ENDIF
	\ENDFOR
	\STATE return $S$.
	%\STATE $\epsilon \leftarrow \sqrt{\frac{2}{3} ln \Delta}$.
   	%\STATE $S(\epsilon) \leftarrow \{ i \in V: v_i \cdot r \ge \epsilon \}$.
   	%\STATE $S'(\epsilon) \leftarrow \{ i \in S(\epsilon): \forall e_{ij} \in E, j \notin S(\epsilon) \}$.
   	%\STATE $S'(\epsilon)$.
\end{algorithmic}
\end{algorithm}



==> doc/futurework.tex <==
% Future works
\section{Future Works}
\label{sec:conclusion}

\subsection{Vertex Cover based Nodes Splitting}

Previous work in \cite{DPL_ICCAD08_Kahng} used a heuristic method to split nodes.
Due to the lack of the entire view, their methods can't guarantee the minimum number of stitches.
\cite{DPL_ICCAD09_Xu} preserve all suitable candidate stitches and didn't pre-slice nodes.
Although this strategy has a entire view, thy dramatically increase the problem size.

We propose a \textbf{Vertex Cover in Hyper-graph}\footnote{Also called "Minimum Hitting Set" problem.} based nodes splitting method.
Our method not only has entire view, but also can decrease the problem size.
(Vertex Cover problem is NP-hard, maybe we can only use ILP or Searching method to solve it ...)

\subsection{Weighted Max Independence Set (MIS) based Coloring Algorithm}

Label each node with different weight. Node that can be easier to move labels low weight.
So the problem is Patterning Decomposition $+$ Layout Modification... (layout modification can only be considered in future work...).

Note that MIS problem is also NP-complete.
Although there are available MIS solvers, it would suffer from runtime penalty if problem size is huge.

\appendices
\section{Other Coloring Algorithms}

\subsection{Dynamic Programming based}

Similar to \cite{kCVM_DAC97Chang}.
Note that 2-Layer assignment is nearly equal to double patterning decomposition, but multi-layer assignment is more complex than multi-patterning decomposition. In multi-layer assignment the order of layers is important, while here order of colors doesn't matter.

\subsection{Optimal algorithm after graph modification}

As discussed before, deciding whether a planar graph is 3-colorable is NP-complete,
but we have following sufficient conditions for a planar graph to be 3-colorable \cite{2003Borodin}:

\begin{conjecture}
\label{conj:1}
Every planar graph without adjacent 3-cycles and without 5-cycles is 3-colorable.
\end{conjecture}

Based on Conjecture.\ref{conj:1}, we can design the following heuristic algorithm:
\begin{enumerate}
    \item{Modify layout to generate graph without adjacent 3-cycles nor 5-cycles.}
    \item{Use SAT solver to solve 3-coloring problem.}
    \item{Heuristically assign color to previous layout.}
\end{enumerate}

==> doc/remove.tex <==
%Step 1:
%   Conflict Detection and Remove
\section{Un-3-Colorable Detection and Remove}
\label{sec:DetectRemove}

\subsection{Un-3-Colorable Detection}

\begin{figure}[thb]
	\centering
	\subfigure[]{
		\includegraphics[width=0.22\textwidth]{FixColor}
	}
	\subfigure[]{
		\includegraphics[width=0.26\textwidth]{ConstraintConflict}
	}
	\caption{(a) Node $a$ and node $d$ must be assigned same color, they are color constraint.
	(b) By transitivity, node $a$ and $f$ are color constraint. Note that node $c$ and $e$ are also color constraint.
	Since $a$ connects $f$, there is color constraint conflict.}
	\label{fig:FixColor}
\end{figure}

Before carrying out three color assignment, it is helpful to detect un-3-colorable sub-graphs in conflict graph. 
Using Lemma \ref{lem:dp3} we know it's impossible to find out all un-3-colorable graphs in polynomial time.
Here we just detect one type of un-3-colorable graph. 
We will show that in practical nearly all un-3-colorable sub-graphs can be found by our detection method.

To help find these un-3-colorable sub-graphs, we define a special relationship between two nodes.

\begin{define}[Color Constraint]
If two nodes must be in same color, they are color constraint.
\end{define}

We call those nodes with color constraint as color constraint nodes.

\begin{lemma}
Two adjacent 3-cycles include two color constraint nodes.
\label{lem:3cycle}
\end{lemma}

As shown in Fig.\ref{fig:FixColor}(a), node $a$ and node $d$ must in same color, they are color constraint nodes.
Besides color constraint is transitive, e.g. in Fig.\ref{fig:FixColor}(b), $a$ and $d$ are color constraint, $d$ and $f$ are color constraint, then $a$ and $f$ are color constraint.


\begin{define}[Color Constraint Conflict]
Two nodes are color constraint conflict, if and only if they are color constraint and connected.
\end{define}

From Fig.\ref{fig:FixColor}(b) we can see node $a$ and node $f$ are color constraint, and there is an edge connecting them.
So $a$ and $f$ are color constraint conflict.
Using Lemma \ref{lem:3cycle} and transitivity, we can iteratively find all color constraint nodes.

\begin{figure} [thb]
  \centering%
    \subfigure[Four-polygon Clique]{%
      \label{fig:4clique}
      \includegraphics[width=0.22\textwidth]{4clique}
    }
   \subfigure[Special cycle]{%
      \label{fig:cycle}
      \includegraphics[width=0.2\textwidth]{cycle}
    }
  \caption{Un-3-colorable graphs in \cite{TPL_SPIE08_Cork} can be detected.}
  \label{fig:detection}
\end{figure}

\begin{figure}[thb]
	\centering
	\includegraphics[width=0.3\textwidth]{UnDetect}
	\label{fig:UnDetect}
	\caption{Our detection method can't detect this un-3-colorable graph \cite{2003Borodin}.}
\end{figure}

Fig.\ref{fig:detection} show that un-3-colorable graphs in \cite{TPL_SPIE08_Cork} can be detected by our methods.
Is there a figure we can't detect? The answer is yes. \cite{2003Borodin} gives an example.
The conflict graph is rare in IC layout, so we ignore detection this type.


\subsection{Un-3-Colorable Remove}

We have two methods to remove conflicts: node split and edge remove. 
Note that node split equals to stitch insertion, and edge remove equals to layout modification.

\begin{lemma}
Four-polygon Clique can only be eliminated by edge remove (layout modification).
\end{lemma}

The simplest method is to remove edge. 
We observe that removing any edge in Fig.\ref{fig:detection}(b) can make the new graph 3-colorable.
However, remove edge means modify layout.
So we prefer to remove un-3-colorable by node splitting.


==> doc/speedup.tex <==
\section{Optimal Speed-Up Techniques}
\label{chap:speedup}


\begin{figure*}[t]
	\centering
	\subfigure[]{
		\includegraphics[width=0.19\textwidth]{input}
	}
	\subfigure[]{
		\includegraphics[width=0.19\textwidth]{Simplify1}
	}
	%\hspace{.1em}
	\subfigure[]{
		\includegraphics[width=0.19\textwidth]{Simplify2}
	}
	%\hspace{.1em}
	\subfigure[]{
		\includegraphics[width=0.19\textwidth]{Simplify3}
	}
	\subfigure[]{
		\includegraphics[width=0.19\textwidth]{Simplify4}
	}
	\hspace{.1em}
	\subfigure[]{
		\includegraphics[width=0.19\textwidth]{Simplify5}
	}
	%\hspace{.1em}
	\subfigure[]{
		\includegraphics[width=0.19\textwidth]{Simplify6}
	}
	%\hspace{.1em}
	\subfigure[]{
		\includegraphics[width=0.19\textwidth]{Simplify7}
	}
	%\hspace{.1em}
	\subfigure[]{
		\includegraphics[width=0.19\textwidth]{Simplify8}
	}
	\subfigure[]{
		\includegraphics[width=0.19\textwidth]{Simplify9}
	}
	\caption{Layout Graph Simplification.~(a)Input layout.~(b)Corresponding layout graph.~(c)(d)(e)Iteratively remove and push in nodes with edges no more than 2.~(f)(g)(h)(i)After color assignment, iteratively pop up and recover node, and assign any legal color.~(j)Final Decomposition result.
	%In this case all nodes can be pushed in stack. If there are some nodes can't be simplified, carry out Color Assignment algorithm.
	}
	\label{fig:Simplify}
\end{figure*}

Since ILP is NP-hard problem, and its runtime increases dramatically when the size of Decomposition Graph is large.
In this section we propose three speed-up techniques to simplify the Layout Graph or Decomposition Graph to reduce time complexity of ILP.
Note that our speed-up techniques are optimal, in other words, ILP formulation can still get optimal solutions.
As shown in Fig.\ref{fig:overview}, our speed-up flow includes three steps: Independent Component Computation, Layout Graph Simplification and Bridges Computation.

\subsection{Independent Component Computation}

We propose independent component computation on decomposition graph for reducing the ILP problem size without losing optimality.
In layout graph of real layout, we observe many isolated occupied clusters.
Therefore, we can break down the whole design into several independent components , and apply basic ILP formulation for each one.
The overall solution can be taken as the union of all the components without effecting the global optimality.
The runtime of ILP formulation scales down dramatically with the reduction of the variables and constraints, and the coloring assignment can be effectively accelerated.




\subsection{Layout Graph Simplification}
\label{sec:Simplification}

We can simplify layout graph by removing all nodes with degree less or equal to two.
At the beginning, all nodes with degree less or equal to two are detected and removed temporarily from Layout Graph.
This removing process will continue untill all the nodes are at least degree-three.
The layout graph simplification algorithm is shown in Algrithm \ref{alg:Simplify}.
Note that our simplification algorithm can minimize ILP problem size drametically.

\begin{algorithm}[htb]
\caption{Layout Graph Simplification and Color Assignment} 
\label{alg:Simplify}
\begin{algorithmic}[1]
   \REQUIRE Layout Graph $G$ to simplified, stack $S$
   \WHILE{$\exists n \in G$ s.t. $degree(n) \le 2$}
         \STATE $S.push(n)$;
         \STATE $G.delete(n)$;
   \ENDWHILE
   \STATE Decomposition graph construction.
   \STATE TPL Decomposition for nodes can not be simplified.
   \WHILE{ $! S.empty()$}
   	\STATE $n = S.pop()$;
	\STATE $G.add(n)$;
	\STATE Assign $n$ a legal color.
   \ENDWHILE
\end{algorithmic}
\end{algorithm}

If all the nodes in layout graph can be simplified (pushed into stack), TPL Decomposition can be solved optimally in linear time. 
An optimal example is shown in Fig.\ref{fig:Simplify}.
Note that even some nodes can not be simplified, layout graph simplification can reduce problem size. 
Besides, we observe that this algorithm can also partition layout graph into several sub-graphs.

Note that this simplification method can not use in decomposition graph. (Add some example...)

%\subsection{Cut Vertex Computation}
%Our cut vertex computation is similar to \cite{DPL_ICCAD2010_Yuan}. But we observe that partition Decomposition Graph by removing Cut Vertex may introducing new stitch, while partition Layout Graph by removing Cut Vertex keep optimality.

%In "Introduction to Algorithm".


\subsection{Bridges Computation}

\begin{figure}[tb]
	\centering
	\subfigure[]{
		\includegraphics[width=0.23\textwidth]{bridge1}
	}
	\subfigure[]{
		\includegraphics[width=0.23\textwidth]{bridge2}
	}
	\hspace{0.1em}
	\subfigure[]{
		\includegraphics[width=0.23\textwidth]{bridge3}
	}
	\subfigure[]{
		\includegraphics[width=0.23\textwidth]{bridge4}
	}
	\caption{Bridges Computation.~(a)Initial decomposition graph.~(b)After bridges computation, remove edge $e_{ab}$.
			~(c)In two sub-graphs carry out ILP formulation.~(d)Rotate colors in right sub-graph to add bridge.
	}
	\label{fig:bridge}
\end{figure}

A bridge of a graph is an arc whose removal disconnects the graph into two components.
Since two new components are independent, partition graph by removing bridge can also partition whole ILP into two independent ILP formulations.
An example of bridges computation is shown in Fig. \ref{fig:bridge}.

\begin{theorem}
Partition Decomposition Graph by removing bridges does not introduce new stitch.
\end{theorem}

We adopt an $O(|V|+|E|)$ algorithm \cite{1974Tarjan} to find bridges in decomposition graph.

